Millimeter Wave Wireless Assisted Robot Navigation with Link State Classification

The millimeter wave (mmWave) bands have attracted considerable attention for high precision localization applications due to the ability to capture high angular and temporal resolution measurements. This paper explores mmWave-based positioning for a target localization problem where a fixed target broadcasts mmWave signals and a mobile robotic agent attempts to capture the signals to locate and navigate to the target. A three-stage procedure is proposed: First, the mobile agent uses tensor decomposition methods to detect the multipath channel components and estimate their parameters. Second, a machine-learning trained classifier is then used to predict the link state, meaning if the strongest path is line-of-sight (LOS) or non-LOS (NLOS). For the NLOS case, the link state predictor also determines if the strongest path arrived via one or more reflections. Third, based on the link state, the agent either follows the estimated angles or uses computer vision or other sensor to explore and map the environment. The method is demonstrated on a large dataset of indoor environments supplemented with ray tracing to simulate the wireless propagation. The path estimation and link state classification are also integrated into a state-of-the-art neural simultaneous localization and mapping (SLAM) module to augment camera and LIDAR-based navigation. It is shown that the link state classifier can successfully generalize to completely new environments outside the training set. In addition, the neural-SLAM module with the wireless path estimation and link state classifier provides rapid navigation to the target, close to a baseline that knows the target location.

==> extra.tex <==

%\paragraph*{TX synchronization beam sweep modeling}  

HERE
To enable detection, we assume the TX transmits a known
synchronization signal, sweeping through a sequence of directions
from the different TX arrays.  Since there are a total of
$N_{\rm ant}^{\rm tx} N_{\rm arr}^{tx}$ antennas at the TX,
we can represent each TX direction by a beamforming vector, 
$\nbw_k^{\rm tx} \in \C^{N_{\rm ant}^{\rm tx} N_{\rm arr}^{tx}}$,
representing the complex phases applied to the different 
antenna elements when transmitting in direction $k$.
We will call each TX beamforming vector $\nbw_k^{\rm tx}$
a \emph{TX codeword} and we
let $N_{\rm cw}$ denote the total number of TX codewords.
The set of TX codewords will be called the (multi-array) codebook.
We will assume that each TX codeword is transmitted on only one
TX array at a time both to conserve power and not assume any local
oscillator synchronization across TX arrays.
We let $T_{\rm SS}$ denote the time for each TX
synchronization signal so the total time to transmit all
$N_{\rm cw}$ is $T_{\rm SS}T_{\rm cw}$.  We assume the beam sweep 
pattern is repeated every $T_{\rm per}$ seconds with 
$T_{\rm per} \geq T_{\rm sig}$

\paragraph*{TX and RX position}
We denote the unknown TX position by
$\nbx^{\rm tx} = (x^{\rm tx}_1, x^{\rm tx}_2, x^{\rm tx}_3)$,
which we will assume is fixed.
For the receiver motion, we will assume 
the time is divided into time steps of length $T$,
In time step $k$, we will denote the receiver position by
$\nbx^{\rm rx}_k = (x^{\rm rx}_{k1}, x^{\rm rx}_{k2}, ^{\rm rx}_{k3})$.
A critical assumption is that the receiver position is exactly known
relative to some reference frame (e.g.\ the starting or end position)
of the robot.  This will be enabled with an IMU under the assumption 
we can ignore the drift.  \textcolor{red}{[SR:  Is this valid?]}



\subsection{Configuration and Synchronization Issues}
The methods described above apply to any scenario where the target device
can transmit a mmWave beam sweeping synchronization signals.
Such signals are commonly used in mmWave RADAR and can be used in this application
if the target can carry a RADAR transmitter.
If the target device has a standard 5G mmWave device, then the existing
management and positioning signals may be used
\cite{giordani2018tutorial,keating2019overview,dwivedi2021positioning},
but some additional configuration capabilities may be needed.
For example, if the target is a 5G UE device, the path estimation could
potentially be performed from
the uplink sounding reference signals (SRS).
The mobile agent could then attempt to listen to the SRS signals for localizing the target.
Of course, normally the SRS are directed to the serving base station.
Hence, 
for the signaling method described above, the UE would need to receive some configuration
from the network to transmit the SRS in a sweeping pattern.  
Also, if the UE does not have a connection to a mmWave
base station (a likely scenario since the target may be inside where the mmWave
signals are blocked), the UE would need to be configured over a sub-6 GHz
carrier and be permitted to transmit even in absence of a detected network.

Whichever signals are used, one issue is the transmit synchronization.
For the mobile target receiver to know the tranmsit angle, $\Omega$

%\subsection{Navigation}
Having extracted the path parameters
and classified the link state,
we can then employ the follow the following
simple navigation strategy:
If the link state is classified as either
LOS or First-Order NLOS, we navigate in the
direction of the strongest RX angle of arrival.
Otherwise, if the link state is classified 
as the either Higher-Order NLOS or Outage,
we assume the navigation system
has an ability to continue to explore the 
environment.  The environmental exploration
can use any method. In the simulations,
we will use the neural SLAM module.


\textcolor{red}{[SR:  Someone describe
this dataset and provide examples of how this
has been used by roboticists.}
\textcolor{blue}{[MY:Start]}
Two data sets are provided: mmWave indoor ray tracing data and mmWave indoor channel sounding data, both of which contain the data needed for robot indoor SLAM and navigation simulation.
The indoor mmWave ray tracing data is a set of noiseless signal propagation path data, which provides the ideal ray tracing paths for each pair of TX-RX in the indoor environment.
An actual propagation path consists of the received power, angle of arrival and departure, propagation time, and the coordinates of the interactions.
On the other hand, the mmWave indoor channel sounding data is generated from the mmWave indoor ray tracing data set.
we implement the comprehensive antenna array modeling, beam sweeping, and path estimation procedures, 
which are shown in \ref{sec:direst} and \ref{sec:algo}.
mmWave indoor channel sounding data set accurately adds noise to make it more realistic and can be used to simulate signals received by robot agents in a real environment.
Importantly, our generated mmWave datasets is perfectly compatible with the original Gibson models, which allows us to easily use the wireless data in Habitat-Sim \cite{habitat19iccv, szot2021habitat} and 
Neural-SLAM \cite{chaplot2020learning} robot simulation platforms.
\textcolor{blue}{[MY:End]}


\subsection{Overview}
In this section, we review the proposed
algorithms for the path estimation
and link state classification:
\begin{itemize}
    \item \emph{Path estimation} detects 
    the paths and estimate their parameters
    including angles, SNRs and delay;
    \item \emph{Link state classification} then estimates
    the link state from the path parameters
\end{itemize}
As we will describe in the robotics simulations
below, the path estimates and link
state will be used as the basis for the 
navigation.


\textcolor{blue}{[MY:Start]}where
$g_\ell$ is the path gain,
$\Omega^{\rm rx}_\ell$ is the angle of arrival,
$\Omega^{\rm tx}_\ell$ is the angle of departure,
and $\tau_\ell$ is the path delay of the path $\ell$.
And $L$ denotes the maximum number of 
paths recorded for a link.
\textcolor{blue}{[MY:End]}
These paths can then
be used in the channel model \eqref{eq:rxsig}.
For each path, the ray tracing describes
its physical route including whether the
paths are LOS or NLOS.  For the NLOS paths,
it indicates the set of all interactions
including diffractions, reflections,and transmissions.
\textcolor{blue}{[MY:Start]}
Fig.\ref{fig:ray_tracing_example} shows part of ray tracing paths of a LOS link and a NLOS link.
In the LOS case, the strongest path is always a direct LOS path, while some NLOS paths also exist.
We cannot be certain that the strongest path will result from a one-time interaction (diffraction, reflection, or transmission) or a multi-time interaction.
We create an indoor ray tracing data set \cite{5g-indoor-github} which stores the ray tracing paths data of all TX-RX links of total 38 unique maps.
As shown in Fig. \ref{fig:map_demostration}, we use a unified RX grid with total 25600 RX locations, since the layouts are different in different maps, the inside-of-room RX locations are different.
In the mmWave indoor ray tracing data set, we only keep the inside-of-room RX links data, and discard the links which outside the room.
To make the robot navigation test simple and uniform on different maps, the data set records the relative coordinates and indexes of each receiver in the room.
Furthermore, the maximum number of accepted paths $L$ of a TX-RX link is set to 25, which abandons paths with very lower received power.
\textcolor{blue}{[MY:End]}



%The 3D indoor models based on the floor-plans created by AI Habitat \cite{savva2019habitat} were imported. A representation is shown in Fig. 2. Transmitters were randomly placed at 10 locations inside the room and the receivers gird were uniformly placed at 25600 locations in the map with a 0.15 meters distance between every two points. The height of both transmitters and receivers are 1.5 meters.

\textcolor{blue}{[MY:Start]}
Following the ray tracing implementation in the indoor environment, the path parameters of the TX-RX links will be utilized to conduct a beam sweeping double direction channel estimation. 
The beam searching and channel sounding result for a link is already defined in \eqref{eq:pathparam}.
After removing the path relative delay, we define the channel sounding link vector
\begin{equation} \label{eq:nn-inputs}
     \mathbf{x} = \left\{
    (\Omegahat_\ell^{\rm rx},
    \Omegahat_\ell^{\rm tx},\gamma_\ell),
    ~ \ell = 1,\ldots, K \right\}
\end{equation}
where $K$ is the number of paths, $\Omegahat_\ell^{\rm rx}$ is azimuth angle of arrival of path $\ell$, 
$\Omegahat_\ell^{\rm tx}$ is azimuth angle of departure of path $\ell$, 
and $\gamma_\ell$ is the SNR of the path $\ell$.
In our simulation, we keep the most strongest 5 paths from the path estimation via low-rank tensor decomposition which means $K=5$
in which case, 
the channel sounding link vector $\mathbf{x}$ contains total $3K = 15$ parameters.
% The mmWave indoor channel sounding data set is similar to the mmWave indoor ray tracing data set.
We store the channel sounding results of the robot agent in all inside-of-room locations of different maps.
In which case, when we test on a specific map
and the robot agent is at a certain position in the room, we can find the correspondent channel sound link vector $\mathbf{x}$ from the date set through 
the coordinates of the agent, the position of transmitter, and the name of the map.
% It is reasonable to use this particular channel sounding link vector $\mathbf{x}$, as the paths that the robot agent actually receives.
\textcolor{blue}{[MY:End]}

For the 
As a result of the TX and RX codebooks we defined in the previous part, we can calculate the MIMO channel response using the knowledge we acquired in section \ref{sec:algo}.
The ray tracing paths data is the input of the standard multi-path cluster model to compute the received signal shown in \eqref{eq:rxsig}.
Some simulation parameters are set as follows:
the transmit power of TX (gNB) is 23 dBm;
the sampling rate is 400 MHz;
the noise figure is 6 dB;
the size of one FFT window is 1024.
For each TX-RX link, based on the ray tracing paths,
we simulate a noise mmWave MIMO channel.
TX sends a synchronization signal along with each TX codeword, and the RX performs beamforming in each RX codeword direction.  
Then the RX performs a match filter on each TX-RX beamforming pair to extract the channel response in that direction. 
Since every path in a link has a different angle of arrival (AoA), angle of departure (AoD), and delay, the beamforming complex gain and relative delay samples are different for each path.
When examining the MIMO channel response of a link, adding all paths, the beam direction is determined by taking the maximum variance of the response along with the delays at each TX-RX beamforming pair.
% The SNR is computed by dividing the maximum by the mean of the variance of the channel responses.  
The SNR can be used for thresholding to determine if there is a peak. 
% Fig. \ref{fig:h_peak} plots the channel response of two links, where we illustrate the SNR in each TX-RX direction pair along with the location of the actual ray tracing paths of links.  


% The beam search provides a coarse estimate of the AoD and AoA.  
% On the other hand, 
% to solve problems like the robot localization and navigation, 
% we need better angular estimates. 
We used an SVD-type algorithm in the simulation to implement the low-rank tensor decomposition discussed in section \ref{sec:algo}, and we recorded the 5 paths with the highest SNR.
As it requires coherent measurements across the antennas in different arrays, this procedure can only be performed at the RX (robot agent).
% In addition, 
% we assume we have a fully digital array at the RX.
By using coherent measurements, a RX scanning codebook with a $1\degree$ resolution is created and used to determine the most correlated AoA angle from scanning codewords


To explore the robot indoor navigation algorithms,
we employ the Habitat AI \cite{habitat19iccv} 
as the robot simulation platform.
Additionally, to handle the navigation decision 
when the robot agent is
locating outside the coverage of wireless signals or 
it thinks the wireless signal is untrustworthy,
we use the Neural-SLAM \cite{chaplot2020learning} 
algorithm.
The Neural-SLAM can do random exploring without
wireless information, ....

\textcolor{blue}{[Akshaj:]





can be easily transferred to point goal navigation task by setting the point goal as the long term goal in the Global policy. In our work, we use these pre-trained Neural SLAM, Global Policy and Local Policy networks for the agent to efficiently navigate through the environment by suitably setting the long-term goal as shown in Fig. \ref{fig:nslam}.

\textcolor{blue}{[MY:]
I'm not sure if we need to explain following detail::::
The way we set the global goal based on AoA periodically is:
set the global goal 15 steps away on the extend line of strongest path's AoA direction.
Here 'step' in '15 steps' is defined by NSLAM system.
The robot need about 12-13 steps to rotate 180\degree.
And in our simulation, the global goal updates in every 15 steps moving.
So if we use the AoA to set the next period gobal goal, 
the robot in general first rotates itself to face toward the AoA direction,
and then walks in some steps in this direction (based on local policy)
(the number of steps depend on how many steps remain after rotating).
I do not modify the local policy.
}



Under the easy level tests, as shown in Figure \ref{fig:arrival_speed}(a), \emph{AoA based on SNR} and  have the same extremely fast speed, where 90\% of the tests are completed in three times the number of steps of the baseline algorithm. 
Contrary to the \emph{AoA when LOS} algorithm, which is less efficient, the main reason for this situation is that when the robot is not in LOS state at the initial position, it will use the Active Neural-SLAM exploring.
The Active Neural SLAM exploring will cause the robot to move away from the destination (TX) with a certain probability.

The results of the test at moderate difficulty are shown in Figure \ref{fig:arrival_speed}(b). In 75 percent of test cases, \emph{AoA based on SNR} and \emph{AoA when LOS or First-order NLOS} have the same speed. 
However, only the \emph{AoA when LOS or First-order NLOS} algorithm was able to complete more than  90\% of the tests using five times as many steps as the baseline algorithm.
Therefore, the robot is more likely to be affected by signal noise as the difficulty of the test increases.
Through this phenomenon, we can know that, in the Higher-order NLOS cases, measuring errors of AoA from path estimation can lead to confusion in the navigation system.

Figure \ref{fig:arrival_speed}(c) illustrates the performance of three algorithms based on hard level cases. 
During the test at the hard difficulty level, it becomes evident that the \emph{AoA when LOS or First-order NLOS} algorithm has a large advantage over the other two algorithms.
When implementing the \emph{AoA when LOS or First-order NLOS}, around 90\% of the hard tests use six times the number of steps of the baseline algorithm.
Due to the effectiveness of the link-states classification neural network, the \emph{AoA when LOS or First-order NLOS} algorithm only uses the measured AoA if the wireless signal is reliable. 
This minimizes the possibility of taking a detour and maximizes the probability of moving the robot towards its target TX.
On the contrary, without the link-states classification neural network, when the robot runs the \emph{AoA based on SNR} algorithm, it always uses the wireless information even if the estimated AoA is not reliable when the link of current location is higher-order NLOS.
It is highly likely that the larger error in angle estimation will result in the robot moving in the wrong direction.
In the meantime, \emph{AoA when LOS} is still slower than \emph{AoA when LOS or First-order NLOS}. 
It follows that if the robot uses AoA to help it navigate only when in LOS, it will lose a substantial amount of reliable information and therefore have to spend more time conducting random explorations.



leveraging the classification of link-states, the robot considers the current position to be in the higher-order NLOS and evaluates the measured wireless information to have high error and low confidence.
Therefore, the robot performs the Active Neural SLAM map exploring. Consequently, the robot is prevented from being trapped in areas where the signal is unreliable.
In this test, the robot with the \emph{AoA when LOS or First-order NLOS} algorithm performs 208 steps better than the robot running on the \emph{AoA based on SNR} algorithm.

On the whole, the millimeter wave wireless-based indoor navigation algorithms that rely on the angle-of-arrival are efficient and reliable.
We implement the mmWave multiple antenna array on both the TX and RX sides, and we also apply the beam sweeping double directional estimation technique so that the robot (RX) can receive the AoD information. 
With both AoD and AoA, a link-states classification neural network can achieve a 90\% accuracy rate. 
Link-state classification of high accuracy allows us to develop a more efficient navigation algorithm, which is \emph{AoA when LOS or First-order NLOS}.
Based on the received wireless signal, the \emph{AoA when LOS or First-order NLOS} algorithm allows the robot to analyze the current link-state situation and decide whether or not to use received path's AoA to guide its next period navigation.
When the robot believes that it is within LOS or first-order NLOS, since the measured wireless data is likely to be credible in such a case, it uses the AoA information to navigate. 
When the robot is in higher-order NLOS or outage situations, the wireless signal is weak and the wireless data being measured has a high probability of lager error due to noise, so it considers using some randomly exploration algorithms.


%To add the state-of-the-art indoor navigation comparison, we tested a fully computer vision-based SLAM navigation algorithm and compared it to our proposed algorithms that utilize wireless signals as an aid.
%On the other hand, Huang and Molisch et al. propose the machine learning based LOS and NLOS identification methods \cite{huang2020machine}.
%We used the static characteristics discussed in their paper as the input to train a two connected layer neural networks, and we compared it with our link-state classification network.

%In the revised manuscript, we highlight our novelties and contributions with our new results.

\begin{itemize}
\item[(i)]
It is true that link state classification between the Line-Of-Sight (LOS) and the Non-Line-Of-Sight (NLOS) has been discussed in wireless communication field,
for example, in paper \cite{huang2020machine}, Huang and Molisch et al. propose the machine learning based LOS and NLOS identification methods for the multiple-input and multiple-output (MIMO) system in vehicle-to-vehicle (V2V) networks. 
It is our novelty to extend the classes of link state classification into three categories: LOS, first-order NLOS, and higher-order NLOS.
The first-order NLOS link is defined as that at least one of the path in this link is only interaction with the environment one time.
For example, if the link includes a one-time reflection path (Transmitter-Reflection-Receiver) or a one-time diffraction path (Transmitter-diffraction-Receiver), the link is a first-order NLOS link.
And in the paper's proposed indoor navigation scenario, our results show that the three-category classifier (LOS, first-order NLOS, and higher-order NLOS) is more useful than the two-category one (LOS and NLOS).

\item[(ii)]	
The path estimation via low-rank tensor decomposition technical can help us find the strongest path of a link. 
In this technical framework, if we consider that we will only use the wireless signal information to design the indoor robot navigation algorithm, it would appear that the state of the art navigation algorithm is the ``AoA based on SNR" algorithm that is presented in this paper.
The ``AoA based on SNR" algorithm is defined as that based on the path estimation results, we use the Angle of Arrival (AoA) of the strongest path whose SNR is higher than a pre-select threshold to set up the moving goal of the next robot operation period. 

\item[(iii)]
The ``Major Changes'' section above contains detailed results of the new tests of the comparison to baseline algorithms for navigation and comparison to prior algorithms for link state detection.

\end{itemize}


%We now provide more explanations concerning the difference between first-order NLOS and higher-order NLOS in this manuscript.
As described in the paper, we consider each ``Transmitter-Receiver'' link including multiple paths.
The LOS link is defined that a link exists a LOS path (transmitter directly to receiver path), and on the contrary, the NLOS link means that a link does not has a LOS path.
The LOS path does not interact with the environment such as walls, floors, ceilings, or furniture.

In contrast, as shown in Fig.~\ref{fig:link-state}, the signal transmission in a NLOS path interacts with the environment by reflecting and diffracting.
The first-order NLOS link and higher-order NLOS link are extended from the definition of the NLOS link.
We use the existence of the one-time interaction path to distinguish the first-order NLOS and higher-order NLOS link.
The first-order NLOS link is defined as that at least one of the path in this link is only interaction with the environment one time.
For example, if the link includes a one-time reflection path (Transmitter-Reflection-Receiver) or a one-time diffraction path (Transmitter-Diffraction-Receiver), the link is a first-order NLOS link.
At the same time, an example of a two-time interaction path can be ``Transmitter-Reflection-Reflection-Receiver'', which means that in this path, the signal reflects on two surfaces before it receives by the receiver. 


We provide pre-trained neural networks, and the robot does not need to retrain a networks for starting a navigation mission.
This is exactly what the navigation tests that we describe in paper section VI do.
There are a total of 38 different maps provided, and each map is unique. 
In the section V, 18 of them were used to train the link-state classification neural network, and then the navigation algorithms were tested on the remaining 20 maps.
Through the 18 maps, the robot obtains a pre-trained model.
It is important to know that the remaining 20 maps are not used when we are training the link-state classification neural network.

We use 20 maps to run the navigation tests, and for the robot, these 20 maps are unknown environments.
During the test, the robot reads the signal from the current position and estimates the paths according to the wireless channel.
Next, the estimated paths are used as input to the pre-trained link-state classification neural network.
It is unnecessary for the robot to retrain its classification neural network at this point.
In navigation, since the robot does not need to retrain the network, it only requires the pre-trained network to predict the current link state, so if the robot equips the pre-trained network before the navigation mission, there is no delay caused by training the network.

==> intro_v2.tex <==
\section{Introduction}
\label{sec:intro}

%{mmwave use for }
5G millimeter wave (mmWave) wireless has 
tremendous potential in enabling new localization technologies~\cite{}.
High precision localization is useful for many 
applications including \todo{...}~\cite{}. In this paper, we investigate the use of mmWave wireless 
for target localization (the target here is a mmWave transmitter) in unmapped indoor environments, 
%and 
%illustrate its use in enabling a mobile robot to navigate to the target location. 
%ine-of-sight (LOS) vs. non line-of-sight (nLOS) classifier that determines the 
aided by a novel line-of-sight (LOS) versus non line-of-sight (NLOS) classifier.  
Distinguishing LOS vs. NLOS is important for localization because of \todo{severe signal attenuation in NLOS settings ~\cite{paper1, paper2}.} 
%paper1: https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=7997068&casa_token=3jBQpQoiQ0UAAAAA:A61E1qIQE6dEGfbGISrMxd-dPhSo1gkP8KsHGm9LOepKT-Oh4LLFcTL8GbgwKwXmSjwHhVZt4A&tag=1
%paper2: https://ieeexplore.ieee.org/abstract/document/8968748?casa_token=zlVwBFDPH58AAAAA:YjBhfEMEWXeA0eZAu5TxHEUhvP5_pnI8JrTILniNE5nQUb7BUokCkC9slsOhLSHPS09vfhtf5A

%Recent years have seen tremendous 
%advances in three parallel
%localization and navigation technologies:
%high resolution camera and LiDAR systems for
%mobile platforms; deep neural network-based  
%simultaneous localization and mapping (SLAM) techniques
%for complex environments; and fifth generation
%(5G) positioning methods based on high frequencies
%transmissions in the millimeter wave (mmWave) bands.
%The combination of these technologies offers
%new opportunities for navigation, exploration
%and localization.
\textcolor{red}{[SR:  Do not know if I like this
intro.  Also needs many references.]}
\textcolor{red}{[SG:  took a stab at rewriting, but still dont like it. missing a key message.]}

In this work, we consider applying these methods
for a target localization and
navigation problem illustrated in Fig.~\ref{fig:problem}:
A fixed target is located at some unknown position
and a mobile agent must locate and navigate to the
target.  We assume the environment and obstacles are not known,
so the agent may need to 
perform simultaneous localization and mapping
(SLAM) within the environment as part of the target discovery. 
\begin{figure}
    \centering
    \includegraphics[width=6cm]{Figures/room_target_agent.png}
    \caption{Target localization and navigation problem.  
    A target has a wireless transponder.  An agent
    must locate and navigate to the target
    using received wireless signals along with
    camera and LiDAR data.}
    \label{fig:problem}
\end{figure}

To assist in the localization and navigation, we assume
that the agent has simultaneous access to two modes
of sensor    data:  Camera / LiDAR data as well
as millimeter wave (mmWave) wireless measurements.
For the wireless measurements, we assume the
target has a wireless transponder that broadcasts
known synchronization signals.  The agent has a wireless
receiver that can detect these signals and estimate their angles
of arrival and receive power to 
assist in the localization of the target.

This localization and navigation can be applied in a range
of application.  Most directly, search and rescue, ...

Our contributions to this problem are as follows:
\begin{itemize}
    \item \emph{Modular localization and navigation algorithm:}  As described in Section~\ref{sec:overview},
    we propose a simple three stage 
    algorithm that separates the wireless directional estimation and visual SLAM.  In the proposed method,
    qt each RX location, the agent 
    first estimates the 
    angles of arrival and SNR of the wireless paths
    from the TX.  Given measurements from multiple RX locations, the agent then attempts to determine
    a valid target location that can be given to 
    a visual SLAM module.    The method is completely modular, allowing
    any wireless directional estimation to be
    integrated 
    into state-of-the-art visual SLAM modules such 
    as \cite{chaplot2020learning}.
    
    \item \emph{Multi-array directional estimation.}
    Since mmWave antenna elements 
    tend to be highly directional, 
    multiple arrays oriented in different directions
    are often required on both the mobile (UE)
    and base station (gNB) to obtain 360 degree coverage
    \cite{raghavan2019statistical,xia2020multi}.
    We describe a novel method for beam search 
    and directional estimation for such multi-array 
    systems (Section~\ref{sec:direst}).  
    Importantly, the methods
    do not require phase coherence across the arrays
    allowing independent local oscillators.
    
    \item \emph{Anchor point estimation and classification}:
    To combine the wireless angles of arrival information
    from multiple RX locations, we propose a novel 
    anchor point estimation algorithm. It is well-known that, in non-line-of-sight (NLOS) environments, 
    the paths to the receiver will appear as arriving from
    a set of ``virtual transmitters" or anchor points
    \cite{olivier2016lightweight}.   We propose a $K$-means
    type algorithm that can determine which paths
    came from which anchor points and then
    find an optimal anchor point that can be used as the
    next target destination.  
    The method also performs a 
    binary classification on whether the
    a valid anchor point for navigation can be found.
    
    \item \emph{Integration with Visual SLAM}:
    The outputs of the anchor point estimation can then
    be readily integrated into any visual SLAM module, 
    including state-of-the-art neural SLAM methods 
    such as \cite{chaplot2020learning}.  
    We assume the visual SLAM module can support two modes:
    an 
    \textbf{exploration mode} where the target location is unknown and the agent simply explores and maps the environment; 
    and \textbf{point-goal task} where the agent 
    has a specific target location.  Given such a module,
    we simply set the agent in exploration mode 
    when a valid anchor point cannot be found and then
    provide the anchor point as the point-goal
    when a valid anchor point is found.
    
    \item \emph{Validation in realistic, complex
    environments:}   The proposed approach is validated 
    on the AI Habitat robotic simulation environment \cite{savva2019habitat} with the Gibson data set \cite{xia2018gibson}.  This environment and dataset 
    have
    a detailed robotic kinematic models along with
    camera and LiDAR data from a large number
    of indoor environments 
    \textcolor{red}{[SR:  provide more details.}
    For the wireless simulation, 
    we augment the dataset with ray tracing
    at \SI{28}{GHz} using state-of-the-art
    ray tracer \cite{Remcom} to 
    predict the wireless propagation in each environment.
    The wireless propagation data is combined
    with realistic models of the arrays and estimation algorithms.  We also show and simulate
    how the wireless localization can be performed
    within the 5G New Radio positioning signaling
    \cite{keating2019overview} -- a key enhancement
    introduced in the latest 3GPP specification.
    
    
    \item \emph{Public dataset:}  All the code
    and wireless data is made public, providing the 
    first complete 5G wireless localization dataset
    combined with camera data and robotic simulation
    environment.  \textcolor{red}{[SR: Describe this better, provide links]}.  
    
\end{itemize}

\subsection*{Prior Work}
The problem has a number of new and interesting features:

\textcolor{red}{[SR:  Discuss what is known in mmWave
and camera localization. Prior positioning methods
assume fixed infrastructure.  Discuss 3GPP positioning
methods.}

% mmWave localization
Nowadays, the indoor positioning technology has not yet converged to a unique perfect method \cite{potorti2021off},
and the mmWave communication systems can be more easily integrated into existing devices, 
such as smart phones and small form factor devices with low power consumption \cite{huo20175g, niu2015survey}.
For the indoor positioning of mmWave wireless systems, 
three important wireless measurement methods based on received signal strength (RSS), 
time difference of arrival (TDoA) and angle of arrival and departure (AoA and AoD) are generally considered \cite{el2014evaluation}.
5G positioning roughly has the following four research directions:
Millimetre-Wave MIMO, Multi-path Assisted, Device-to-Device Communication Enables Cooperative Positioning in Ultra-Dense Networks, 
and Hybrid Fusion of Multiple Sensor \cite{del2017survey}.
Millimetre-Wave MIMO is the foundation of the AoA and AoD based positioning algorithm, 
because the 5G antenna allows the generation of highly directional beams between the transmitter and receiver, while the high attenuation loss limits the number of reflections that reach the multi-path \cite{roh2014millimeter, guerra2015position, shahmansoori20155g, guidi2014millimeter}.
Multi-path Assisted localization allows to reduce the needed infrastructure and makes the single fixed anchor positioning possible \cite{witrisal2016high}.
On the other hand, in 5G mmWave propagation, it is crucial to determine if a multi-path link includes a Line-Of-Sight path. ...........

% 3GPP
\textcolor{red}{[Ming:How detailed do this part need?].}
3GPP standard documents provide a detailed definition of the positioning function and implementation in the 5G New Radio (5G NR) scenario.
For indoor scenarios, the target horizontal positioning requirements for commercial use cases studied in Rel-16 were $<$3 m (80\% UEs).\cite{3GPP38885}. 
The more recent 3GPP Rel-17 \cite{3GPP38857} proposes a new goal for commercial use requirements is $<$ 1 m for 90\% of UEs.
3GPP Rel-16 \cite{3GPP21916} has specified various location technologies for the 5G NR to support regulatory as well as commercial use cases. 
In general, there are three major categories: Radio access technology (RAT)-dependent, RAT independent, and combination of RAT-dependent and RAT-independent techniques.
Evaluation results have shown that in indoor scenarios it is feasible to achieve commercial target performance requirement for horizontal positioning accuracy using RAT-dependent solutions. 
For the uplink (UL) based positioning, UL-TDOA and UL-AoA based positioning techniques are widely used.
To improve the performance and stability of positioning, 
the combination of downlink (DL) and uplink (UL) based positioning is taken into account,
which integrates TDOA, UL-AoA, and DL-AoD techniques \cite{3GPP38885}.
For example, under the conditions of the 3GPP standard test, with carrier frequency 30 GHz and transmission bandwidth 400 MHz, the HiSilicon, Huawei combined the UL and DL data and used the enhanced cell identity (E-CID \cite{wigren2007adaptive}) positioning algorithm to achieve the error $\leq$ 1.0 m for 90\% UEs and $\leq$ 0.6 m for 80\% UEs in the indoor open office scenario \cite{3GPP38885, 3GPP-R1-1901577,3GPP-RAN1-Taipei}.

% Camera





==> intro_v3.tex <==
\section{Introduction}
\label{sec:intro}

%{mmwave use for }
5G millimeter wave (mmWave) wireless has 
tremendous potential in enabling new localization technologies~\cite{}.
High precision localization is useful for many 
applications including \todo{...}~\cite{}. In this paper, we investigate the use of mmWave wireless 
for target localization (the target here is a mmWave transmitter) in unmapped indoor environments, 
%and 
%illustrate its use in enabling a mobile robot to navigate to the target location. 
%ine-of-sight (LOS) vs. non line-of-sight (nLOS) classifier that determines the 
aided by a novel line-of-sight (LOS) versus non line-of-sight (NLOS) classifier.  
Distinguishing LOS vs. NLOS is important for localization because of \todo{severe signal attenuation in NLOS settings ~\cite{paper1, paper2}.} 
%paper1: https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=7997068&casa_token=3jBQpQoiQ0UAAAAA:A61E1qIQE6dEGfbGISrMxd-dPhSo1gkP8KsHGm9LOepKT-Oh4LLFcTL8GbgwKwXmSjwHhVZt4A&tag=1
%paper2: https://ieeexplore.ieee.org/abstract/document/8968748?casa_token=zlVwBFDPH58AAAAA:YjBhfEMEWXeA0eZAu5TxHEUhvP5_pnI8JrTILniNE5nQUb7BUokCkC9slsOhLSHPS09vfhtf5A

%Recent years have seen tremendous 
%advances in three parallel
%localization and navigation technologies:
%high resolution camera and LiDAR systems for
%mobile platforms; deep neural network-based  
%simultaneous localization and mapping (SLAM) techniques
%for complex environments; and fifth generation
%(5G) positioning methods based on high frequencies
%transmissions in the millimeter wave (mmWave) bands.
%The combination of these technologies offers
%new opportunities for navigation, exploration
%and localization.
\textcolor{red}{[SR:  Do not know if I like this
intro.  Also needs many references.]}
\textcolor{red}{[SG:  took a stab at rewriting, but still dont like it. missing a key message.]}

In this work, we consider applying these methods
for a target localization and
navigation problem illustrated in Fig.~\ref{fig:problem}:
A fixed target is located at some unknown position
and a mobile agent must locate and navigate to the
target.  We assume the environment and obstacles are not known,
so the agent may need to 
perform simultaneous localization and mapping
(SLAM) within the environment as part of the target discovery. 
\begin{figure}
    \centering
    \includegraphics[width=6cm]{Figures/room_target_agent.png}
    \caption{Target localization and navigation problem.  
    A target has a wireless transponder.  An agent
    must locate and navigate to the target
    using received wireless signals along with
    camera and LiDAR data.}
    \label{fig:problem}
\end{figure}

To assist in the localization and navigation, we assume
that the agent has simultaneous access to two modes
of sensor    data:  Camera / LiDAR data as well
as millimeter wave (mmWave) wireless measurements.
For the wireless measurements, we assume the
target has a wireless transponder that broadcasts
known synchronization signals.  The agent has a wireless
receiver that can detect these signals and estimate their angles
of arrival and receive power to 
assist in the localization of the target.

This localization and navigation can be applied in a range
of application.  Most directly, search and rescue, ...

Our contributions to this problem are as follows:
\begin{itemize}
    \item \emph{Multi-array directional estimation.}
    Since mmWave antenna elements 
    tend to be highly directional, 
    multiple arrays oriented in different directions
    are often required on both the mobile (UE)
    and base station (gNB) to obtain 360 degree coverage
    \cite{raghavan2019statistical,xia2020multi}.
    We describe a novel method for beam search 
    and directional estimation for such multi-array 
    systems (Section~\ref{sec:direst}).  
    Importantly, the methods
    do not require phase coherence across the arrays
    allowing independent local oscillators.
    
    \item \emph{Anchor point estimation and classification}:
    To combine the wireless angles of arrival information
    from multiple RX locations, we propose a novel 
    anchor point estimation algorithm. \todo{we are not using anchor points in NLOS setting, I thought it is just for LOS...modified the text accordingly}
    %It is well-known that, in non-line-of-sight (NLOS) environments, 
    %the paths to the receiver will appear as arriving from
    %a set of ``virtual transmitters" or anchor points
    %\cite{olivier2016lightweight}.   
    We propose a $K$-means
    type algorithm that can determine which paths
    came from which anchor points and then
    find an optimal anchor point that can be used as the
    next target destination.  
    %The method also performs a 
    %binary classification on whether the
    %a valid anchor point for navigation can be found.
    
    \item \emph{Integration with Visual SLAM}:
    The outputs of the anchor point estimation can then
    be readily integrated into any visual SLAM module, 
    including state-of-the-art neural SLAM methods 
    such as \cite{chaplot2020learning}.  
    We assume the visual SLAM module can support two modes:
    an 
    \textbf{exploration mode}, which is invoked in NLOS setting, where the target location is unknown and the agent simply explores and maps the environment; 
    and \textbf{point-goal task} where the agent 
    has a specific target location based on anchor point estimation in LOS settings. 
    Given such a module,
    we simply set the agent in exploration mode 
    when a valid anchor point cannot be found and then
    provide the anchor point as the point-goal
    when a valid anchor point is found.
    
    \item \emph{Validation in realistic, complex
    environments:}   The proposed approach is validated 
    on the AI Habitat robotic simulation environment \cite{savva2019habitat} with the Gibson data set \cite{xia2018gibson}.  This environment and dataset 
    have
    a detailed robotic kinematic models along with
    camera and LiDAR data from a large number
    of indoor environments 
    \textcolor{red}{[SR:  provide more details.}
    For the wireless simulation, 
    we augment the dataset with ray tracing
    at \SI{28}{GHz} using state-of-the-art
    ray tracer \cite{Remcom} to 
    predict the wireless propagation in each environment.
    The wireless propagation data is combined
    with realistic models of the arrays and estimation algorithms.  We also show and simulate
    how the wireless localization can be performed
    within the 5G New Radio positioning signaling
    \cite{keating2019overview} -- a key enhancement
    introduced in the latest 3GPP specification.
    
    
    \item \emph{Public dataset:}  All the code
    and wireless data is made public, providing the 
    first complete 5G wireless localization dataset
    combined with camera data and robotic simulation
    environment \cite{5g-indoor-github}.  
    \textcolor{red}{[SR: Describe this better, provide links]}.
    The dataset consists of two parts: 5G indoor ray tracing data, 
    and channel modeling with beam search results.
    \textcolor{red}{[Ming: Should we give a summary of the data set here
     and write the detail explaination in a single section?].}
    % To generate 28 GHz indoor ray tracing dataset, 
    % we employ a powerful ray tracing package, Wireless InSite by Remcom \cite{Remcom}. 
    % The 3D indoor models based on the floor-plans created by AI Habitat were imported. 
    % A representation is shown in Fig. \ref{fig:remcom_map_demostration}. 
    % Transmitters were randomly placed at ten locations inside the room and the receivers gird were uniformly placed at 25600 locations in the map with a 0.15 meters distance between every two points. The height of both transmitters and receivers are 1.5 meters.
    % The ray tracer produces the maximum 25 number of paths for a TX-RX link.
    % There are  received  
    
    
    
\end{itemize}

\begin{figure}
  \centering
  \includegraphics[width=0.6\linewidth]{Figures/remcom_map.jpg}
  \caption{A example of ray tracing simulation area representing a 24m $\times$ 24m region of a indoor environment. Ten green dots represent transmitter locations and a red dots grid represents the receiver grid. (The ceiling of room is not shown.)}
  \label{fig:remcom_map_demostration}
\end{figure}



\subsection*{Prior Work}
The problem has a number of new and interesting features:

\textcolor{red}{[SR:  Discuss what is known in mmWave
and camera localization. Prior positioning methods
assume fixed infrastructure.  Discuss 3GPP positioning
methods.}

% mmWave localization
Nowadays, the indoor positioning technology has not yet converged to a unique perfect method \cite{potorti2021off},
and the mmWave communication systems can be more easily integrated into existing devices, 
such as smart phones and small form factor devices with low power consumption \cite{huo20175g, niu2015survey}.
For the indoor positioning of mmWave wireless systems, 
three important wireless measurement methods based on received signal strength (RSS), 
time difference of arrival (TDoA) and angle of arrival and departure (AoA and AoD) are generally considered \cite{el2014evaluation}.
5G positioning roughly has the following four research directions:
Millimetre-Wave MIMO, Multi-path Assisted, Device-to-Device Communication Enables Cooperative Positioning in Ultra-Dense Networks, 
and Hybrid Fusion of Multiple Sensor \cite{del2017survey}.
Millimetre-Wave MIMO is the foundation of the AoA and AoD based positioning algorithm, 
because the 5G antenna allows the generation of highly directional beams between the transmitter and receiver, while the high attenuation loss limits the number of reflections that reach the multi-path \cite{roh2014millimeter, guerra2015position, shahmansoori20155g, guidi2014millimeter}.
Multi-path Assisted localization allows to reduce the needed infrastructure and makes the single fixed anchor positioning possible \cite{witrisal2016high}.
On the other hand, in 5G mmWave propagation, it is crucial to determine if a multi-path link includes a Line-Of-Sight path. ...........

% 3GPP
\textcolor{red}{[Ming:How detailed do this part need?].}
3GPP standard documents provide a detailed definition of the positioning function and implementation in the 5G New Radio (5G NR) scenario.
For indoor scenarios, the target horizontal positioning requirements for commercial use cases studied in Rel-16 were $<$3 m (80\% UEs).\cite{3GPP38885}. 
The more recent 3GPP Rel-17 \cite{3GPP38857} proposes a new goal for commercial use requirements is $<$ 1 m for 90\% of UEs.
3GPP Rel-16 \cite{3GPP21916} has specified various location technologies for the 5G NR to support regulatory as well as commercial use cases. 
In general, there are three major categories: Radio access technology (RAT)-dependent, RAT independent, and combination of RAT-dependent and RAT-independent techniques.
Evaluation results have shown that in indoor scenarios it is feasible to achieve commercial target performance requirement for horizontal positioning accuracy using RAT-dependent solutions. 
For the uplink (UL) based positioning, UL-TDOA and UL-AoA based positioning techniques are widely used.
To improve the performance and stability of positioning, 
the combination of downlink (DL) and uplink (UL) based positioning is taken into account,
which integrates TDOA, UL-AoA, and DL-AoD techniques \cite{3GPP38885}.
For example, under the conditions of the 3GPP standard test, with carrier frequency 30 GHz and transmission bandwidth 400 MHz, the HiSilicon, Huawei combined the UL and DL data and used the enhanced cell identity (E-CID \cite{wigren2007adaptive}) positioning algorithm to achieve the error $\leq$ 1.0 m for 90\% UEs and $\leq$ 0.6 m for 80\% UEs in the indoor open office scenario \cite{3GPP38885, 3GPP-R1-1901577,3GPP-RAN1-Taipei}.

% Camera
\textcolor{blue}{[>>>> APT: Added prior work for :
Los/NLoS classification and SLAM]}
\\
\textbf{LoS and NLoS Identification}
\\
WiFi based applications such as activity recognition, indoor localization, gesture recognition, etc need the awareness of the receiver presence in LoS or NLoS. NLoS signal propagation can result in a large amount of noise and multipath effect, thus, deteriorating the quality of the communication link further lowering the accuracy of the application. Some solutions employ the use of extremely wide-band signals such as Ultra Wide Band (UWB) \cite{guvenc2007nlos, venkatesh2007non,khodjaev2010survey}. UWB has a large bandwidth so, LoS signals can be easily identified and extracted with the help of propagation delay, range measurements, and other channel statistics. However, these UWB LoS and NLoS techniques cannot be extended to WiFi networks because of narrower bandwidth and absence of detailed precise feature measurements as in UWB. Some have proposed techniques that use the Multiple Input Multiple Output(MIMO) techniques with a large number of antennas \cite{xiong2013arraytrack, } but they either need hardware for measuring angular spectra or sophisticated correlation techniques, thus, limiting their scope of practical use. 

There have been several prior work that exploit the Channel State Information (CSI) or PHY layer features such as phase delays \cite{zhou2014lifi} or phase features \cite{wu2015phaseu} but \cite{zhou2014lifi} needs extracted CSI to be converted into time domain CIR and \cite{wu2015phaseu} explores both space diversity and frequency diversity along with the use of special instruments such as gyroscopes making it costly. \cite{xiao2014non} use multiple features from RSS samples, \cite{Han teal et al} use SVM on features extracted from a group of RSS and RTT samples, but these techniques use fixed sampling rate and analyze more accessible signal features from multiple packets that not only adds to high cost and time but also degraded real-time performance. Also, the techniques that use PHY layer CSI need driver modification. Additionally, a lot of these techniques have been tested on same or similar maps so we do not know how well they perform on a never before seen map.

Our technique for LoS and NLoS identification needs collection of n samples at a point that is fed to the 2-layer Neural Network thus avoiding the need for collection of large samples of data to identify LoS v/s NLoS. Additionally, our classifier demonstrates demonstrates high accuracy for never before seen indoor spaces. 

\textbf{Localization and Mapping:}
Localization and Mapping:
Indoor location based services comprise of 2 parts - (i) Mapping module, that is responsible for the physical map of the indoor space and (ii) Localization module, that is responsible for identifying the position on the indoor map. 

The task of Localization has been widely studied by both the robotics and the networking community and the methods can be broadly divided into 2 main types - device free and device based. Device free localization methods do not need the person or object that is localized to carry any device. In this method \cite{} we commonly equip the environment with sensors that help perform localization. However, device free techniques require installation of sensors resulting in high installation and maintenance cost and cannot be easily universally adopted. On the other hand, device based methods need the human or object localized to carry along a device. With the ubiquity of WiFi indoors, we have a lot of promising WiFi based indoor localization methods \cite{}. Fingerprinting based methods work in offline and online mode. First, in the offline model they perform data collection of the Received Signal Strength (RSSI) and generate a fingerprinted map of various RSSI values at multiple locations on the indoor map. Next, in the online phase for realtime localization, they collect the RSSI values at the current location and map them to the closest fingerprinted location \cite{joydeep, etc}. Fingerprinting based methods are labor intensive, need the indoor floor map knowledge in the offline phase and the modifications to the floor map needs to be incorporated manually. Some techniques use Channel State Information (CSI) such as \cite{Array..} or accurate Time of Flight information as in \cite{}, resulting in hardware modification making these methods hard to deploy. RSSI based techniques such as \cite{} use triangulation techniques where RSSI values from multiple Access Points (AP) are used to locate the device/human. These techniques are easy to deploy but have an error of 2-4 meters. Our proposed approach uses RSSI values to identify LoS v/s NLoS paths but we differ from the above techniques ***fill in this sentence***.

Recently with the advancement in Neural Networks there have been some research on using neural networks for localization such as \cite{} that use measured wireless channel values as inputs to the neural network either directly or after transformation into images with the goal to localize the device. A lot of these methods use complex CSI information that is not easily acquirable without any modification or the method used is computation heavy and not easily interpretable.

\textcolor{blue}{[ <<<<< APT: End of text]}


==> overview.tex <==
\section{Overview of the Proposed Localization and
Navigation Algorithm}
\label{sec:overview}

We propose a simple joint localization  and navigation 
strategy based on three steps:
\begin{itemize}
    \item \emph{Directional estimation:}  First, for each
    RX location, the RX attempts to estimate the paths
    from the TX to the RX.  The path estimates will include
    the number of sufficiently strong paths (if any),
    and for each path, its 
    RX angle, RX power and relative delay.  
    As discussed below,
    if certain additional synchronization assumptions
    can be made, estimates of 
    the TX angles and absolute delay
    may also be available.
    
    \item \emph{Waypoint Estimation:}  Next, 
    given path estimates
    at multiple RX locations, the problem is to attempt
    to locate the TX or, a valid waypoint to the TX.
    Since mmWave signals have limited range, a valid waypoint
    may not always be available.
    Critical in our design is that, in addition to
    waypoint estimation, is that we determine if
    a valid waypoint can be found.
    
    
    \item \emph{Navigation:}  Based on waypoint
    
\end{itemize}


==> prior.tex <==

\subsection*{Prior work}
The works \cite{guvenc2007nlos, venkatesh2007non,khodjaev2010survey} consider
LOS/NLOS detection using delay spread measurements in UWB systems.  
However, these do not incorporate angular measurements, which are key
in any mmWave context.  More recently, 
\cite{huang2020machine} incorporated angular measurements for vehicular systems at
\SI{5.9}{GHz}.  This work used 
MIMO sounding enables precise AoD and AoA measurements.  In contrast, this work assumes only TX side beam sweeping, and therefore can be implemented in 
mmWave transmitters with analog beamformers.  They key challenge with beam sweeping is that the TX angles are only coarsely resolved.

\cite{wang2018pursuance} mmWave positioning in NLOS with
anchors using AoA.  No AoD.

\cite{guerra2018single}  CRB for single path beamforming 
and MIMO.  No beam sweeping.

\cite{lu2020positioning} LOS positioning from a single UL 
antenna.

\cite{kim20185g} positioning from single TX and RX of 
a vehicle in motion.  Assumes abstracted measurement model
where the path parameters are recieved plus noise.

\cite{guvenc2007nlos} uses simple hypothesis testing.
Delay only.
